GDPevo: Evaluating Agent Self-Evolution on Real Business Tasks

Agent self-evolution updates an agent's persistent state from prior experience and reuses it to solve related tasks more effectively. Evaluating self-evolution is difficult: existing benchmarks provide limited coverage of economically valuable task domains, do not always design training and test tasks such that test-time gains can be attributed to training experience, and remain vulnerable to data contamination. We present GDPevo, an evolution-native benchmark grounded in GDP-related enterprise workflows, together with the fully automated data pipeline that generates it. Its core mechanism, rule hybridization, decomposes each enterprise workflow into atomic business rules, distributes subsets of these rules across training tasks, and recombines them in held-out test tasks so that test-time gains are attributable. GDPevo spans CRM, ERP, finance, healthcare, legal, and data-centric workflows. Its V1 release contains 120 tasks in 12 groups, with five training and five held-out test tasks per group. Full automation enables the pipeline to expand the suite to 240 tasks in 24 groups (V2) within two days, providing a practical response to contamination. Using GDPevo, we evaluate four agents, each comprising a harness and a model, under four supervision types. Self-evolution consistently improves held-out accuracy by up to 16.44 percentage points. But the best evolved agents remain far below the fully informed oracle ceiling of 91.6%, indicating that the self-evolution ability of current agents remains far from fully realized. We publicly release the pipeline, benchmark, and full evaluation results at https://github.com/Prism-Shadow/GDPevo.

==> figs/fig-eval-ablation.tex <==
\begin{figure}[t]
\begin{center}
% ============================================================
% PLACEHOLDER FIGURE --- data not yet collected.
% Replace the framed box below with the rendered PDF once the
% rule-hybridization ablation in Section~\ref{sec-eval} is run.
% ============================================================
\setlength{\fboxsep}{0pt}%
\fbox{\parbox[c][4.6cm][c]{0.92\columnwidth}{\centering
\placeholder{\textbf{[Placeholder: rule-hybridization validity]}}\\[4pt]
\placeholder{Grouped bars, one cluster per task group.}\\
\placeholder{$x$: train-set coverage condition}\\
\placeholder{$\{$all-rules-present, one-rule-held-out,}\\
\placeholder{rules-shuffled-across-groups$\}$.}\\
\placeholder{$y$: test \acck. Expected pattern: accuracy}\\
\placeholder{degrades monotonically as the held-out test}\\
\placeholder{tasks require rules that were removed from}\\
\placeholder{or corrupted in the train set --- evidence that}\\
\placeholder{the test set measures \emph{recombination}, not memorization.}
}}
\caption{\textbf{(To be completed.)} Rule-hybridization validity ablation. We will re-run each task group under three train-set conditions while holding the test set fixed: \emph{(i)} the released train set (all atomic rules present but scattered), \emph{(ii)} one atomic rule withheld from every train task, and \emph{(iii)} train rules randomly permuted across task groups (so train ``experience'' is irrelevant to the test). If \bench truly measures self-evolution by recombination, then \fewshot/\reflect accuracy should drop sharply under \emph{(ii)} and collapse toward the \base level under \emph{(iii)}, while \base accuracy is unchanged. This experiment isolates generalization from memorization and is the key internal-validity check for the benchmark. \emph{Data for this ablation is not yet in the released repository (see Section~\ref{sec-eval-gaps}).}}
\label{fig-eval-ablation}
\end{center}
\vskip -0.2in
\end{figure}


==> figs/fig-eval-transfer.tex <==
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.92\columnwidth]{figs/figs/fig-eval-transfer.pdf}}
\caption{Cross-domain transfer matrix (Claude Code harness). Cell $(x,y)$ is the test \acck\ obtained by \emph{evolving on the train tasks of group $x$ and then testing on group $y$}; we report it as the lift over the in-distribution \base of group $y$. The \textbf{diagonal} is the released in-group result of Section~\ref{sec-eval-q1} (numbers shown, colored by lift); the \textbf{off-diagonal} cells (hatched) require new runs and are not yet collected. Light separators mark the CRM / ERP / Finance domain blocks. We expect a strong diagonal with off-diagonal cells near or below zero: if evolving on the \emph{wrong} group does not help (and sometimes hurts), the gains are attributable to learning each group's specific hidden rules --- a second, independent check on rule hybridization (Section~\ref{sec-bench-hybrid}) beyond the ablation of Figure~\ref{fig-eval-ablation}. \emph{Data for the off-diagonal is not yet in the released repository (Section~\ref{sec-eval-gaps}).}}
\label{fig-eval-transfer}
\end{center}
\vskip -0.2in
\end{figure}


==> tables/tbl-construction.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lc}
\toprule
\textbf{Construction-quality metric} & \textbf{Value} \\
\midrule
Candidate task groups generated            & \placeholder{[N/A]} \\
Adopted task groups ($\geq 5/6$ votes)     & 12 \\
Overall acceptance rate                    & \placeholder{[N/A]} \\
Mean reviewer pass votes (of 6)            & \placeholder{[N/A]} \\
Rejected: structure check failed           & \placeholder{[N/A]} \\
Rejected: hidden rule not planted          & \placeholder{[N/A]} \\
Rejected: insufficient difficulty gap      & \placeholder{[N/A]} \\
Mean atomic rules per task group           & \placeholder{[N/A]} \\
Mean difficulty gap (post-evo $-$ \base), calibration & \placeholder{[N/A]} \\
\bottomrule
\end{tabular}
\caption{\textbf{(To be completed.)} Construction-quality statistics for the automated \bench pipeline. These numbers quantify how selective the multi-agent factory is and substantiate the claims that the pipeline ``outruns data leakage'' and is ``scalable.'' The released repository currently reports only the 12 \emph{adopted} task groups; the generation/rejection counts, reviewer-vote distribution, and calibration difficulty gaps are not yet logged (see Section~\ref{sec-eval-gaps}). We recommend instrumenting Stages~2--3 to emit these counters during construction.}
\label{tbl-construction}
\end{table}


==> tables/tbl-main.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{llcccccc}
\toprule
\textbf{Harness} & \textbf{Model (setting)} & \textbf{Creator} & \textbf{\base} & \textbf{\fewshot} & \textbf{$\Delta$} & \textbf{\reflect} & \textbf{$\Delta$} \\
\midrule
Codex & GPT-5.5 (xhigh) & Codex & 46.72 & 64.91 & $+18.19$ & 57.45 & $+10.73$ \\
Claude Code & Opus 4.8 (xhigh) & Claude Code & 49.11 & 70.90 & $+21.79$ & 62.72 & $+13.62$ \\
Claude Code & GLM-5.2 (max) & Claude Code & 47.73 & 69.55 & $+21.83$ & 63.35 & $+15.62$ \\
Claude Code & Kimi K2.6 (enabled) & Claude Code & 25.14 & 30.48 & $+5.34$ & 32.68 & $+7.54$ \\
Claude Code & DeepSeek V4 Pro (max) & Claude Code & 46.06 & 54.80 & $+8.74$ & 49.22 & $+3.16$ \\
\bottomrule
\end{tabular}
\caption{V1 test accuracy (\%), averaged over 12 task groups. Each group contains 5 test tasks, and each task is run three times. $\Delta$ is the absolute percentage-point gain over the same agent's \base score. An agent is the harness--model composition; the creator column identifies the harness that distills the training experience into a skill. Skill-creator versions remain \texttt{TODO}.}
\label{tbl-main}
\end{table}


==> tables/tbl-positioning.tex <==
\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccc}
\toprule
\textbf{Benchmark} & \makecell{\textbf{GDP /}\\\textbf{business}} & \makecell{\textbf{Self-}\\\textbf{evolution}} & \makecell{\textbf{Leakage-}\\\textbf{resistant}} & \makecell{\textbf{Rule-based}\\\textbf{+ cost}} \\
\midrule
GDPval~\citep{patwardhan2025gdpval}      & \cmarkx & \xmarkx & \xmarkx & \xmarkx \\
SOP-Bench~\citep{nandi2025sopbench} & \cmarkx & \xmarkx & \xmarkx & \xmarkx \\
$\tau$-bench~\citep{yao2024taubench} & \pmarkx & \xmarkx & \xmarkx & \pmarkx \\
GAIA~\citep{mialon2024gaia}          & \xmarkx & \xmarkx & \xmarkx & \xmarkx \\
AgentBench~\citep{liu2024agentbench} & \pmarkx & \xmarkx & \xmarkx & \xmarkx \\
\midrule
\textbf{\bench (ours)}         & \cmarkx & \cmarkx & \cmarkx & \cmarkx \\
\bottomrule
\end{tabular}
\caption{Positioning of \bench against representative agent benchmarks. \cmarkx/\pmarkx/\xmarkx\ denote full/partial/no support. To our knowledge, \bench is the first benchmark to target agent \emph{self-evolution} on economically valuable (GDP-related) business tasks, with a leakage-resistant train/test split (rule hybridization, Section~\ref{sec-bench-hybrid}) and deterministic rule-based grading that treats accuracy and cost as equally important.}
\label{tbl-positioning}
\end{table}

